Stereo Vision-Based Fall Prediction and Detection using Human Pose Estimation on the AMD Kria K26 SOM

Background and Objective: Falls among elderly people can cause serious injury and reduce quality of life. Timely prediction and detection are essential to prevent harm and support well-being. We propose a portable, low-power, battery-operated, vision-based fall prediction and detection system using HPE on an AMD Kria K26 System-on-Module (SOM). The objective is a non-intrusive, privacy-preserving system for real-time fall detection. Methods: The system uses an Intel RealSense D455 range-sensing camera connected to the K26 SOM by USB. It captures synchronized RGB and depth frames, 640 x 480 x 3 and 640 x 480 pixels, at 60 FPS. The SOM runs a three-stage pipeline with quantized YOLOX, Anchor-to-Joint (A2J), and fall-detection models. YOLOX identifies human bounding boxes from RGB frames, then discards the RGB frames to preserve privacy. A2J uses depth frames to estimate 15 joint keypoints per person. A CNN uses selected joint coordinates (x, y, z) to classify fall activity. YOLOX was trained on CrowdHuman; A2J on ITOP, MP-3DHP, UR Fall Detection, and a custom SDSU PSG dataset; and the CNN on UR Fall Detection and SDSU PSG. The design used a single-core DPU with a serial pipeline and a dual-core DPU running YOLOX and A2J with multiple threads. Results: Quantized accuracy was evaluated using IoU >= 50% for YOLOX, mAP with a 10-cm rule for A2J, and classification accuracy, (TP + TN)/(TP + TN + FP + FN), for the CNN. Accuracies were 74%, 84.13%, and 75.85%. Throughput improved from 2.5 FPS for the single-threaded pipeline to 4.5 FPS for the multi-threaded version. Conclusion: Results demonstrate the feasibility of privacy-preserving fall detection on an AMD Kria K26 edge device. On-device HPE and fall classification runs without cloud dependency, supporting elderly monitoring and assistive healthcare. Future work will improve model accuracy and speed.

==> 3_literature_survey.tex <==
The evolution of fall detection technologies has witnessed a significant shift towards wearable sensors and the incorporation of advanced sensor technologies for improved accuracy and efficiency in detecting falls \cite{Li2009}. Initially, fall detection systems predominantly focused on binary fall detection using different machine and deep learning algorithms. However, recent advancements have explored non-binary cases, considering factors like fall direction and severity.
Accelerometers and gyroscopes have been widely used in wearable fall detection systems to monitor movements and detect falls based on acceleration and angular velocity data \cite{Li2009}. The integration of gyroscope sensors alongside accelerometers has been investigated to enhance fall detection accuracy. The utilization of deep learning algorithms, particularly Convolutional Neural Networks (CNN), has shown promising results in improving the classification accuracy of fall detection systems \cite{Li2017,Hwang2017}.
The shift towards edge computing and machine learning applications on wearable devices has enabled complex computations to be performed directly on the device, leading to more efficient fall detection methods \cite{Mrozek2020,ElAttaoui2020}. Developments in microcontroller units (MCUs) have provided the computational power necessary to implement advanced algorithms on wearable devices, facilitating real-time fall detection capabilities.

\subsection{Existing Approaches and Technologies}
Vision-based systems have gained significant attention due to their non-intrusive nature and ability to capture rich contextual information \cite{Espinosa2019,Bevilacqua2014}. These systems leverage computer vision technologies to analyze human motion \cite{Merrouche2017} and posture \cite{Tran2021}, enabling the identification of potential falls.
RGB camera-based methods rely on traditional computer vision techniques, such as background subtraction, object tracking, and motion analysis, with a combination of machine learning models to detect falls \cite{Huang2018}. However, these methods can be sensitive to lighting conditions, occlusions, and variations in clothing or appearance.
Depth camera-based methods utilize depth sensing technologies to capture 3D information about the scene. These methods analyze the 3D human pose and motion patterns to detect falls \cite{Solbach2017}, often leveraging machine learning techniques for accurate classification. Depth cameras offer advantages in terms of robustness to lighting conditions and occlusions, as well as the ability to capture more detailed information about body posture and positioning.
To address privacy concerns, researchers have explored privacy-preserving techniques, such as obfuscating or anonymizing visual data, as well as leveraging depth information instead of color images to maintain user privacy \cite{Liu2020,pmlr-v116-asif20a}.

\subsection{Challenges and Limitations}
Existing vision-based fall detection and prediction systems face several challenges and limitations, hindering their widespread adoption and real-world deployment.
Ensuring high accuracy and reliability in fall detection and prediction is a primary challenge. False positives and false negatives can lead to unnecessary interventions or severe consequences, respectively. Factors contributing to accuracy and reliability issues include occlusions, variations in human body shapes and sizes, diverse environmental conditions, and the complexity of human movements and postures. The presence of multiple individuals or overlapping activities can further complicate the detection and prediction process \cite{Rajagopalan2017,Igual2013}.
Real-time performance is crucial for timely intervention and injury prevention. However, the computational complexity of vision-based techniques, especially those involving deep learning algorithms for human pose estimation and activity recognition, can pose challenges in achieving real-time performance, particularly on resource-constrained devices or embedded systems. Striking a balance between accuracy and performance remains a significant challenge, requiring efficient algorithms, hardware acceleration, and optimized implementations \cite{Torti2018,Chen2021,Bagal2012}.
The deployment and scalability of vision-based fall detection and prediction systems present unique challenges. These systems often require careful calibration and configuration based on the specific environment and use case. Ensuring consistent performance and reliability across diverse deployment scenarios is a critical issue that needs to be addressed \cite{Zhang2015,Igual2013}.
Vision-based systems are susceptible to various environmental and contextual factors that can affect their performance, such as lighting conditions, occlusions, and cultural norms. Accounting for diverse user preferences, privacy concerns, and cultural sensitivities is essential for widespread acceptance and adoption.
d

==> 4_methodology.tex <==
\subsection{System Overview}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/system_overview.png}
    \caption{The proposed fall detection method. First, a human subject in a frame is detected using YOLOX. Second, the A2J model is applied on the depth frame to estimate the joint pose information. Third, a CNN model analyses a set of frames' joint information to detect the occurrence of fall events. Images are taken from the UR Fall Detection dataset.}
    \label{fig:system_overview}
\end{figure*}
Figure \ref{fig:system_overview} shows the overview of the proposed fall prediction and detection system. The system is comprised of an Intel\textsuperscript{\textregistered} RealSense\textsuperscript{\tiny\texttrademark} D455 range-sensing camera connected to a AMD\textsuperscript{\tiny\textregistered} Kria\textsuperscript{\tiny\texttrademark} KV260 Vision AI development platform. The camera produces frames at a resolution of $640 \times 480$ pixels and a frame rate of 60 frames per second (fps), allowing the system to process and operate in real time. RGBD frames from the camera are processed through a combination of machine learning models on the KV260 to predict the event of a human fall. \\
Upon the availability of a synchronized frameset, the RGB frame is first extracted and provided as input to the YOLOX model for human detection. This model processes the full RGB image and returns bounding box coordinates delineating any detected human subjects in the pixel space, taking the form [\textit{xmin, ymin, width, height}] within the frame dimensions. With humans localized in the scene, the depth frame is subsequently extracted from the frameset and preprocessed to isolate the region of interest using the estimated boundary box. This depth crop is then passed to the A2J pose estimation model which outputs a list of 15 joint coordinates for each detected human in 3D space as [\textit{x, y, z}] triplets. Finally, the predicted joint positions are analyzed by the fall prediction model to categorize the pose as either a fall event, or normal posture, through binary classification~\cite{10388590}.
% The following sections provide a detailed account of the methodology, encompassing data acquisition, human pose estimation, fall detection, and system optimization for the AMD Kria K26 SOM platform.
\subsection{Data Acquisition}
The data acquisition process involves capturing synchronized RGB and depth frames using an Intel\textsuperscript{\tiny\textregistered} RealSense\textsuperscript{\tiny\texttrademark} D455 depth camera. This camera employs active infrared stereo vision technology to generate depth information, enabling the system to perceive the 3D spatial characteristics of the scene. The depth camera captures frames at a resolution of $640 \times 480$ pixels and a frame rate of 60 frames per second (fps), facilitating real-time processing.
The librealsense SDK \cite{realsenseSDK} is employed to interface with the depth camera, enabling seamless color and depth video streaming, as well as providing intrinsic and extrinsic calibration information. This SDK also offers synthetic streams, such as pointclouds and depth alignment to color frames, along with built-in support for recording and replaying streaming sessions in the ROSBag file format.

\subsection{Kria KV260 Vision AI Platform}
The AMD\textsuperscript{\tiny\textregistered}~Kria\textsuperscript{\tiny\texttrademark}~KV260 Vision AI development platform is a powerful and efficient edge computing solution designed for accelerating deep learning and computer vision applications. At the heart of this platform lies the Xilinx Kria K26 System-on-Module (SOM), which combines a quad-core Arm Cortex-A53 CPU with a dual-core Arm Cortex-R5 real-time processor and a dedicated deep learning processing unit (DPU).

The DPU, based on the Xilinx Deep Learning Processor (DLP) architecture, provides hardware acceleration for convolutional neural networks (CNNs), enabling high-performance and energy-efficient inference at the edge. The Kria KV260 platform is well-suited for applications requiring real-time processing of visual data, making it an ideal choice for the proposed fall prediction and detection system.

\subsection{Machine Learning Models}
The fall detection system leverages three main machine learning models: YOLOX for human detection, Anchor-to-Joint Regression Network (A2J) for human pose estimation\cite{a2j}, and a Convolutional Neural Network (CNN) for fall detection and classification. These models are briefly summarized as follows:

\subsubsection{YOLOX}
The primary goal is to detect humans within the camera's field of view, achieved through the utilization of the YOLOX-S object detection model. The YOLOX model is an anchor-free approach known for its exceptional speed and accuracy, requiring fewer operations during inference compared to anchor-based models like YOLOv3~\cite{yolov3} and YOLOv4~\cite{yolov4} . 
Several modifications were made to the model architecture: The activation function was changed from MISH to LeakyReLU, the maxpool sizes of the spatial pyramid pooling (SPP) were changed to 3$\times$3, 5$\times$5, and 7$\times$7, as the DPU has a maximum kernel size of 8$\times$8. Lastly, the number of output labels was limited to only one, i.e., a single person. The YOLOX model was trained on the \textit{CrowdHuman} dataset~\cite{crowdhuman}, a large dataset of human detection images. The primary evaluation metric for object detection is Average Precision (AP) for the person class, representing how accurately the model detects persons. Intersection over Union (IoU) is a key component in calculating AP. It measures the overlap between the predicted bounding box $B_p$ and ground truth box $B_{gt}$:
\begin{figure}[htbp]
\centering
\includegraphics[width=0.1\textwidth]{Figures/iou.png}
\caption{Intersection of Union Concept}
\label{fig:iou}
\end{figure}
$$IoU = \frac{\text{Area of Intersection } (B_p \cap B_{gt})}{\text{Area of Union } (B_p \cup B_{gt})}$$
A prediction is considered a true positive if its IoU with the ground truth exceeds a threshold like 0.5. The IoU directly indicates localization accuracy for object detection. Maximizing IoU typically improves mAP as higher overlap with ground truth equates to better detection performance. The model produces the boundary box coordinates in the format [\textit{xmin, ymin, width, height}], where \textit{xmin, ymin} are the left-top corner of the bounding box. The modified YOLOX model is able to achieve good accuracy on real-time streams from the depth camera.

\subsubsection{Human Pose Estimation}
Accurate human pose estimation is a crucial component of the fall prediction and detection system. This work leverages the Anchor-to-Joint Regression Network (A2J) \cite{a2j}, a deep learning model that infers 3D human body pose from a single depth image. The A2J model employs a 2D CNN ResNet-50 architecture~cite{resnet50} pretrained on the ImageNet dataset \cite{ILSVRC15}~as the backbone network, enabling efficient operation on the resource-constrained Kria K26 SOM platform as all the layers are supported by the DPU architecture.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.25\textwidth]{Figures/skeleton.png}
    \caption{Full human body pose joints of interest.}
    \label{fig:skeleton}
\end{figure}
The A2J model is trained on multiple datasets, including ITOP \cite{itop}, MP-3DHP \cite{mp3dhp}, UR Fall Detection \cite{urfall}, and a custom SDSU\textunderscore PSG dataset. The model predicts the positions of 15 key joints in the human body, represented as 3D coordinates in the camera space.
\subsubsection{Fall Detection and Classification}
The fall detection and classification component of the system utilizes a Convolutional Neural Network (CNN) model \cite{fallDetectorModel} to analyze the predicted 3D human pose information from the A2J model. This CNN model is trained on the UR Fall Detection Dataset \cite{urfall} and the custom SDSU\textunderscore PSG dataset, comprising sequences of falls and activities of daily living (ADL).
The CNN model processes the temporal sequence of 3D joint positions and classifies each frame as either a "fall" or "non-fall" event. The model's performance is evaluated using a confusion matrix, enabling the calculation of essential metrics such as precision, recall, and F1 score, providing a comprehensive assessment of its accuracy in distinguishing between fall and non-fall events.

\subsection{Model Quantization and Deployment}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/deploymentSteps.png}
    \caption{Steps involved in the model development of the pre-trained FP32 PyTorch\texttrademark~AI models into INT8 for inference on the Kria\texttrademark~K26 SOM.}
    \label{fig:deploymentSteps}
\end{figure}
The Vitis AI framework from AMD is leveraged to optimize and deploy the deep learning models on the Kria KV260 platform, taking advantage of its hardware acceleration capabilities. The key components of the Vitis AI stack involved in system optimization workflow are:
\begin{enumerate}
    \item Model Inspector: Before quantizing the pre-trained float model, it is examined with the Vitis AI Model Inspector, which returns partition information showing which operators may operate on which device (DPU/CPU).
    \item Model Quantization: The Vitis AI Quantizer lowers processing complexity without sacrificing prediction accuracy by converting 32-bit floating-point (FP32) weights and activations to 8-bit fixed-point integers (INT8). The pre-trained FP32 PyTorch models (YOLOX, A2J, and Fall Predictor CNN) are quantized to INT8 precision using the Vitis AI Quantizer tool.
    \item Model Compilation: The quantized INT8 models are compiled using the Vitis AI Compiler, which generates an optimized executable model (xmodel file) tailored for efficient execution on the Kria K26 SOM's DPU hardware.
    \item Application Integration: The compiled xmodel is integrated into the software application running on the PetaLinux operating system using the VART (Vitis AI RunTime) APIs. This includes deserializing the xmodel, creating DPU runners, managing input/output tensors, and asynchronous job execution on the DPU.
    \item Runtime Optimization: During inference, the application leverages the VART APIs to optimally utilize the DPU hardware acceleration capabilities. This includes techniques like asynchronous job submission, multi-threading, and efficient data transfer between the CPU and DPU.
\end{enumerate}




==> 5_hardware_software_design.tex <==
\subsection{Deep Learning Processor Unit}
The AMD\textsuperscript{\textregistered} Kria\textsuperscript{\tiny\texttrademark} K26 SOM features a Deep Learning Processing Unit (DPU), a customizable compute engine tailored for convolutional neural networks. The \verb|DPUCZDX8G|, designed for the UltraScale\small{\texttt{+}} MPSoC, seamlessly integrates into the programmable logic (PL) and establishes direct connectivity to the processing system (PS) through an AXI interconnect \cite{dpuProductGuide}. Upon reset, instructions are fetched from off-chip memory to govern the computing engine's operations, with these instructions generated by the Vitis AI compiler for optimized model layer performance.

\subsection{Integrating the DPU into Custom Platforms}
Two primary workflows are supported for integrating the DPUCZDX8G: the Vivado flow and the Vitis flow \cite{dpuWorkflow}. In this research, the Vivado flow was chosen, which involves creating a hardware platform project in Vivado, configuring the hardware for an accelerated design, synthesizing, and generating a bitstream file.

\subsection{Possible DPU Architectures on the KV260}
The AMD\textsuperscript{\textregistered} Kria\textsuperscript{\tiny\texttrademark}~K26 SOM's programmable logic offers various logical resources, including 256K system logic cells, 64 UltraRAM blocks, 144 block RAM blocks, and 1.2K DSP slices. These resources enable the synthesis of different DPU architectures within the programmable logic fabric. The available DPU configurations range from a single high-performance core to multiple lower-performance cores, catering to diverse computational requirements. For instance, a single core B4096 architecture can be implemented, capable of executing 4096 multiply-accumulate (MAC) operations per clock cycle at a frequency of 325 MHz. Alternatively, multiple homogeneous cores can be instantiated, such as two B1600 cores or three B1024 cores, enabling parallel execution of multiple models or workloads.

\subsection{Chosen DPU Architecture}
To achieve optimal system throughput, three distinct hardware architectures were explored and evaluated:
\begin{enumerate}
    \item \textbf{Single-core B4096 DPU design:}
The single-core B4096 architecture allows for the sequential execution of AI models on the DPU. With the maximum available logical resources, this architecture executes 4096 multiply-accumulate (MAC) operations per clock cycle at 325 MHz, providing a higher inference time per model execution. The throughput can be further boosted by employing data parallelism and multi-threading techniques for the DPU runners.
While the single-core design has limited parallel processing capacity, which may impact throughput in scenarios demanding simultaneous model execution, its higher performance per core and the ability to leverage data parallelism and multi-threading make it a compelling choice for our application.
    \item \textbf{Dual-core B1600 DPU design:}
The dual-core B1600 architecture features two homogeneous B1600 DPU cores connected to the Zynq UltraScale+ MPSoC processing system (PS) through an AXI interconnect. This design allows for the parallel execution of models, with YOLOX and A2J running on dedicated DPU cores, while the fall prediction model is executed on the CPU itself.
The dual-core approach offers enhanced throughput by processing input data concurrently on separate cores. However, it introduces potential challenges in balancing the workload between cores and introduces overhead due to offloading the fall prediction model to the CPU.
    \item \textbf{Three-core B1024 DPU design:}
The three-core B1024 architecture allocates separate B1024 DPU cores to each of the three models: YOLOX, A2J, and fall prediction. This design enables parallel execution of all three models, potentially improving overall throughput.
However, the limitations in the operations capability of the B1024 architecture DPU core lead to poor inference results for the computationally intensive YOLOX model. Achieving a balance between model complexity and the available core resources becomes crucial in this scenario.
\end{enumerate}

\subsection{Resource Utilization}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/resource_utilization_4096.png}
    \caption{FPGA Resource Utilization of the 1 core B4096 DPU Design.}
    \label{fig:resourceUtilization_4096}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/resource_utilization_1600.png}
    \caption{FPGA Resource Utilization of 2 core B1600 DPU Design.}
    \label{fig:resourceUtilization_1600}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/resource_utilization_1024.png}
    \caption{FPGA Resource Utilization of the 3 core B1024 DPU Design.}
    \label{fig:resourceUtilization_1024}
\end{figure}
Figures \ref{fig:resourceUtilization_4096}, \ref{fig:resourceUtilization_1600}, and \ref{fig:resourceUtilization_1024} summarize the logical resource utilization for the different DPU architectures explored.

\subsection{Embedded Linux, PetaLinux}
PetaLinux is an embedded Linux Software Development Kit (SDK) targeting
FPGA based system-on-chip (SoC) designs. The PetaLinux SDK contains everything
necessary to build, develop, test, and deploy embedded Linux systems. The PetaLinux
Board Support Package for the KV260 Starter Kit is used to build the embedded Linux to run on the KV260. Kernel is configured to enable the DPU device driver. Root filesystem is configured to include Vitis AI librarries and other supporting library packages within the build image. PetaLinux includes U-Boot, Linux kernel, Device Tree, and Root Filesystem components.

\subsection{Device Tree}
The device tree is a data structure used to describe the hardware components and their connections in a system. Using the XSCT (Xilinx Software Command-line Tool) command \verb|createdts| a device tree domain is created based on the hardware description specified by the \verb|XSA| file (hardware design). The \verb|-overlay| option is used to generate an overlay, which allows for dynamic device tree modifications without rebuilding the entire tree.

\subsection{Accelerated Application}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/acceleratedApplication.png}
    \caption{List of accelerated application available for execution.}
    \label{fig:acceleratedApplication}
\end{figure*}
To dynamically enable the accelerated applications on the AMD Kria K26 SOM we use the platform management utility called \verb|xmutil|. Figure \ref{fig:acceleratedApplication} shows the list of available applications

==> 6_system_design.tex <==
\subsection{Software Architecture}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/prodCons.png}
    \caption{Producer-Consumer Software Architecture}
    \label{fig:prodCons}
\end{figure}
The proposed fall prediction and detection system is implemented using a producer-consumer software architecture, as illustrated in Figure \ref{fig:prodCons}. This architecture decouples the data acquisition process (producer) from the data processing and analysis tasks (consumer), enabling better concurrency, scalability, and fault tolerance.

\subsection{Data Acquisition and Preprocessing}
The producer process is responsible for acquiring data from either a pre-recorded video file or directly from the Intel RealSense D455 camera. The RealSense SDK \cite{realsense} is installed on the AMD Kria KV260 Vision AI Development Platform running PetaLinux, enabling seamless integration with the depth camera. The producer reads synchronized RGB and depth frames at a resolution of $640\times 480$ pixels and a frame rate of 60 fps, facilitating real-time processing.
To ensure data integrity during inter-process communication, header and trailer bytes are used as decorators to identify the start and end of frame data. The producer writes the frame data to a named pipe (FIFO) with a resized buffer to accommodate the large frame size. Semaphores are employed for synchronization, preventing race conditions and ensuring the integrity of data transfer between the producer and consumer processes.

\subsection{Serial Pipeline Implementation} \label{sec:serial-pipeline}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/serialPipeline.png}
    \caption{Serial Design Implementation.}
    \label{fig:serialPipeline}
\end{figure}
The serial pipeline design, as depicted in Figure \ref{fig:serialPipeline}, processes data sequentially using a single-core B4096 Deep Learning Processing Unit (DPU) architecture. The consumer process follows these steps:
\begin{enumerate}
    \item Read frame data from the FIFO pipe.
    \item Extract color and depth frames from the frame buffer.
    \item Run the YOLOX model \cite{yolox} for human detection on the color frame.
    \item If a person is detected, run the A2J model \cite{a2j} for pose estimation on the depth frame using the bounding box coordinates from YOLOX.
    \item Run the fall detection model \cite{fallDetectorModel} on the pose estimation output to classify the pose as a fall or non-fall event.
\end{enumerate}

\subsection{Parallel Pipeline Implementation} \label{sec:parallel-pipeline}
\begin{sidewaysfigure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{Figures/mutlithreadedApplication.png}
    \caption{Parallel Design with Multi\-threaded Implementation.}
    \label{fig:mutlithreadedApplication}
\end{sidewaysfigure}
The parallel design implementation, shown in Figure \ref{fig:mutlithreadedApplication}, utilizes a multi-threaded approach and executes each AI model on a dedicated DPU core. A dual-core B1600 DPU architecture is synthesized, with YOLOX and A2J running on separate DPU cores, and the fall predictor model executing on the ARM CPU.

The main thread enqueues color and depth frames to a shared queue. The YOLOX thread continuously checks for frames in the queue, runs the YOLOX model on the color frame, and enqueues the depth frame and bounding box results for the pose estimation thread. The A2J thread dequeues depth frames, runs the pose estimation model, and passes the pose results to the fall prediction model for classification.

\subsection{Data Logging and Performance Monitoring} \label{sec:data-logging}
To monitor system performance and log relevant metrics, a signal handler is implemented to handle the \verb|SIGALRM| signal. The signal handler function is called periodically (every 100 milliseconds) by the system timer and logs various metrics to a CSV file, including timestamps, frame counts, frame rates, model inference times, and prediction outputs. This logging mechanism enables comprehensive analysis and evaluation of the system's performance.
